On the genus two skein algebra

We study the skein algebra of the genus 2 surface and its action on the skein module of the genus 2 handlebody. We compute this action explicitly, and we describe how the module decomposes over certain subalgebras in terms of polynomial representations of double affine Hecke algebras. Finally, we show that this algebra is isomorphic to the $t=q$ specialisation of the genus two spherical double affine Hecke algebra recently defined by Arthamonov and Shakirov.

==> svg-macros.tex <==
% !TEX root=./main.tex
\makeatletter
\ifdefined\svgpath
% - Dynamically render images
\svgpath{{images/}{}}%
\newcommand{\myincludesvggroup}[4]{%
\renewcommand\svg@ink@area{}%
  \includesvg[#1,#2,inkscapename=#3-#4,inkscapeopt=-i\space#4\space-j]{#3}%
  \renewcommand\svg@ink@area{-C}%
}%
\else
% - Use prerendered images
% \newcommandx{\myincludesvg}[2][1=\linewidth,addprefix=\protected]{%
%     \def\svgwidth{#1}%
%     \import{svg-inkscape/}{#2_svg-tex.pdf_tex}%
% }%
% \newcommandx{\myincludesvgnolatex}[2][1=\linewidth,addprefix=\protected]{%
%     \includegraphics[width=#1]{svg-inkscape/#2_svg-raw.pdf}%
% }%
% /Users/julietcooke/Documents/SphericalDAHAs/
% /Users/julietcooke/Documents/SphericalDAHAs/
\newcommand{\svgroot}[0]{.}
\newcommand{\myincludesvg}[3]{\includegraphics[#1]{\svgroot/svg-inkscape/#3_svg-raw.pdf}}%
\newcommand{\myincludesvggroup}[4]{\includegraphics[#1]{\svgroot/svg-inkscape/#3-#4_svg-raw.pdf}}%
\fi
\makeatletter

%Test
% \svgpath{{/Users/julietcooke/Documents/SphericalDAHAs/images/}{}}
% \newcommand{\myincludesvg}[3]{\includesvg[#1,#2]{#3}}
% \makeatletter
% \newcommand{\myincludesvggroup}[4]{
% \renewcommand\svg@ink@area{}%
% \includesvg[#1,#2,inkscapename=#3-#4,inkscapeopt=-i #4 -j]{#3}%
% \renewcommand\svg@ink@area{-C}%
% }
% \makeatother

 %To load statically generated images
% \newcommand{\myincludesvg}[3]{\includegraphics[#1]{images_png/#3_svg-raw.png}}
% \newcommand{\myincludesvggroup}[4]{\includegraphics[#1]{images_png/#3-#4_svg-raw.png}}

\newcommand{\myincludesvgink}[3]{\myincludesvg{#1}{#2}{#3}}
\newcommand{\myincludesvggroupink}[4]{\myincludesvg{#1}{#2}{#3}{#4}}

\newcommand{\diagramhh}[5]{
\raisebox{-#3}{\myincludesvggroup{scale=#5}{inkscape=nolatex,inkscapeformat=pdf,inkscapename=#1-#2,inkscapeopt=-i #2 -j}{#1}{#2}}\hspace{#4}%
}
\newcommand{\diagramhhink}[5]{
\raisebox{-#3}{\myincludesvggroup{scale=#5}{inkscape=nolatex,inkscapeformat=pdf,inkscapename=#1-#2,inkscapeopt=-i #2 -j}{#1}{#2}}\hspace{#4}%
}
\newcommand{\smalldiagram}[2]{\diagramhh{#1}{#2}{18pt}{0pt}{0.75}}
\newcommand{\mediumdiagram}[2]{\diagramhh{#1}{#2}{20pt}{0pt}{0.75}}
\newcommand{\diagram}[2]{\diagramhh{#1}{#2}{23pt}{0pt}{0.75}}
\newcommand{\smallresult}[2]{\diagramhh{#1}{#2}{21pt}{0pt}{0.75}}
\newcommand{\skeindiagram}[1]{\diagramhh{skeinrelations}{#1}{10pt}{1pt}{0.25}}

